Magnitude-squared coherence: A powerful tool for disentangling Doppler planet discoveries from stellar activity

If Doppler searches for earth-mass, habitable planets are to succeed, observers must be able to identify and model out stellar activity signals. Here we demonstrate how to diagnose activity signals by calculating the magnitude-squared coherence $\hat{C}^2_{xy}(f)$ between an activity indicator time series $x_t$ and the radial velocity (RV) time series $y_t$. Since planets only cause modulation in RV, not in activity indicators, a high value of $\hat{C}^2_{xy}(f)$ indicates that the signal at frequency $f$ has a stellar origin. We use Welch's method to measure coherence between activity indicators and RVs in archival observations of GJ 581, alpha Cen B, and GJ 3998. High RV-H$\alpha$ coherence at the frequency of GJ 3998 b, and high RV-S index coherence at the frequency of GJ 3998 c, indicate that the planets may actually be stellar signals. We also replicate previous results showing that GJ 581 d and g are rotation harmonics and demonstrate that alpha Cen B has activity signals that are not associated with rotation. Welch's power spectrum estimates have cleaner spectral windows than Lomb-Scargle periodograms, improving our ability to estimate rotation periods. We find that the rotation period of GJ 581 is 132 days, with no evidence of differential rotation. Welch's method may yield unacceptably large bias for datasets with $N < 75$ observations and works best on datasets with $N > 100$. Tapering the time-domain data can reduce the bias of the Welch's power spectrum estimator, but observers should not apply tapers to datasets with extremely uneven observing cadence. A software package for calculating magnitude-squared coherence and Welch's power spectrum estimates is available on github.

==> Input/computation.tex <==

The Lomb-Scargle method \cite{lomb76, scargle81} is the gold-standard technique for estimating power spectra from irregularly sampled processes. When the spectrum is red, i.e., it has a large amount of low-frequency power, as is the case for many physical processes (such as turbulence), it is common to prewhiten the data by removing an autoregressive model of order one from the time series before assigning significance to the peaks \cite{olafsdottir16}. 

When the number of data points is large, Lomb-Scargle periodograms can be approximated 
by employing an ``extirpolation"
process (interpolation of the unevenly spaced points onto a regular grid) using the
Lagrange interpolation method, and then using the ordinary FFT \cite{press1989fast}.
%However, as described in \cite{leroy2012fast} \cite{springford20},
%one can employ the adjoint nonuniform FFT \cite{keiner2009using} for a fast
%implementation which is not approximate. 

%Briefly, one computes 
%\begin{align}
%S_y &= \sum_i (x_i - \bar{x}) \sin \omega t_i, 
%\quad & C_y &= \sum_i (x_i - \bar{x}) \cos \omega t_i, \\
%S_2 & = \sum_i \sin 2 \omega t_i, 
%\quad & C_2  &= \sum_i \cos 2 \omega t_i,
%\end{align}
%then
%\begin{align}
%\sum_i (x_i - \bar{x}) \cos\omega(t_i - \tau) &= C_y \cos \omega\tau + S_y \sin \omega\tau, \\
%\sum_i (x_i - \bar{x}) \sin\omega(t_i - \tau) &= S_y \cos \omega\tau - C_y \sin \omega\tau, \\
%\sum_i \cos 2  \omega(t_i - \tau) & = \frac{N}{2} + \frac{1}{2} C_2 \cos 2\omega\tau + \frac{1}{2}
%S_2 \sin 2\omega\tau,\\
%\sum_i \sin 2 \omega(t_i - \tau) &= \frac{N}{2}  - \frac{1}{2} C_2 \cos 2\omega\tau - \frac{1}{2}
%S_2 \sin 2\omega\tau.
%\end{align}

==> Input/estimation.tex <==
\subsection{Spectrum and Coherence Estimation}
\label{subsec:estimation}

\cite{lomb76} and \cite{scargle82} developed a method for estimating the power spectrum
when the time series is sampled unevenly. Suppose that $N$ samples of a zero-mean stationary process, $\bfx = [x_0, \ldots, x_{N-1}]^T$, are available on the nonuniform temporal grid, $t_j$ $j= 0,\ldots,N-1$.
One computes the following modified nonuniform Fourier transform 
% The so-called Lomb-Scargle Fourier transform, in Olafsdottir 2016, but this is not the way it is commonly known
 \begin{equation} \label{eq:LSFT}
   \mathcal{F}\{\bfx\}(f) = \frac{\sum_j x_j \cos 2\pi f (t_j - \tau)}{\sqrt{2\sum_j \cos^2 2 \pi f (t_j - \tau)} } + i \frac{ \sum_j x_j \sin 2\pi f (t_j - \tau)}{\sqrt{ 2\sum_j \sin^2 2 \pi f (t_j - \tau)}}
\end{equation}
where the sums over $j$ are from $0, \ldots, N-1$ and the frequency-dependent time offset, $\tau$, is the solution to
\begin{equation} \label{eq:tau}
  \tan 4 \pi f \tau = \frac{ \sum_j \sin 4 \pi f t_j}{\sum_j \cos 4 \pi f t_j}.
\end{equation}
Note that the denominators of both terms in \eqref{eq:LSFT} are approximately $\sqrt{N}$, exact when there is constant $\Dt_j = t_{j} - t_{j-1}, \quad j = 1, \ldots, N-1$. An alternate normalization, and the one we use here \cite{ZK09} is

Finally, the Lomb-Scargle normalized periodogram is
 \begin{equation} \label{eq:LSPgram}
   P_x(f) = \left|\mathcal{F}\{\bfx\}(f)\right|^2.
\end{equation}
When the mean is nonzero, one generally substitutes $x_j - \frac{1}{N} \sum_j x_j$ for the 
original process in the above. The periodogram may be normalized by $1/s_x^2$ where
\begin{equation}
 s^2_x = \frac{1}{N-1} \sum_{j=0}^{N-1} x_j^2 
\end{equation}
is the estimated variance of the process. 

The Lomb-Scargle periodogram of Eqn. \eqref{eq:LSPgram}, despite being a gold-standard estimator for 
the spectrum, has provably poor statistical properties \cite{pw93}. (a) It is a biased estimator of $S_x(f)$, 
and can be shown to be biased, by several orders of magnitude in some cases, even when the sampling 
increments are constant and the spectrum is smooth. Bias is introduced through $\EV P_x(f) \} = (S_x * G)(f)$, where $*$ denotes convolution and $G(f)$ is the spectral window specific to the sampling $t_j$. 
One would prefer that $G(f)$ be delta-like, however it is impossible to create a window function whose
Fourier transform is a delta function, so the result is that power from far-away frequencies tends to
\emph{leak} into the frequency bins of interested by virtue of having been convolved with the window function. (b) The periodogram is inconsistent, that is, $\Var S_x(f) \}$ does not decrease as $N\rightarrow \infty$.
\SDR{I replaced window function with spectral window - usually astronomers use window function to mean the (possibly Fourier transformed) dates and times of observations, not the Fourier transform of a taper}

To decrease bias for spectra and cross spectra, \emph{tapering} is recommended. A data taper is a 
sequence $\bfv = [v(t_0), \ldots, v(t_{N-1})]^T$, which is multiplied by the data
in order to constrain spectral leakage. Denoting the componentwise product $\bfx \otimes \bfv = [x(t_0)v(t_0), \ldots, x(t_{N-1})v(t_{N-1})]^T$, we have the \emph{direct} cross-spectral estimate
\begin{equation} \label{eq:Crosspec}
    \widehat{S}_{xy}(f) = \mathcal{F}\{\bfx \otimes \bfv \}(f)\mathcal{F}^{*}\{\bfy \otimes \bfv \}(f).
\end{equation}
If $v_j = 1/\sqrt{N}$ for all $j$, then $\widehat{S}_{xx}(f) = P_x(f)$---i.e.\ the cross-spectrum of $\bfx$ with {\it itself} becomes the Lomb-Scargle periodogram.

To compute the coherence, however, one cannot simply divide tapered cross spectrum estimates \eqref{eq:Crosspec} by the square roots of the spectra 
$P_x(f)$ and $P_y(f)$ since this results in the
disastrous coherence estimate which is identically one \cite{brockwelldavis92,storchz99}. 
There are two ways to avoid this: (1) to smooth across frequency and
(2) to divide the data into segments and use an averaging approach, 
which we describe in what follows. 
Both of these methods result in decreased resolution of the estimate and so the amount of 
smoothing or number of segments must be chosen with some care. 

\begin{enumerate}
\item Smoothed estimates of MSC, denoted
$\bar{c}^2(f)$, and phase, denoted $\bar{\phi}(f)$ \cite{shumwaystoffer} are computed first by choosing
a suitable smoothing window of length $0 < 2m+1 \ll N$, denoted $h_k, k = -m, \ldots, 0, \ldots, m$
% $h_j, j = -m, \ldots, 0 ,\ldots, m$ 
and computing the smoothed estimates
\begin{align} \label{eq:PgramCoh}
% \bar{S}^h_{x,y}(f) &= \frac{1}{\sqrt{s_x^2 s_y^2}} \sum_{j = -m}^{m} h_j \mathcal{F}\{\bfx \otimes \bfv \}(f -f_j) \mathcal{F}^{*}\{\bfy \otimes \bfv \}(f-f_j) \\
\bar{S}^h_{xy}(f) &= \frac{1}{\sqrt{s_x^2 s_y^2}} \sum_{k = -m}^{m} h_k \mathcal{F}\{\bfx \otimes \bfv \}(f -f_k) \mathcal{F}^{*}\{\bfy \otimes \bfv \}(f-f_k) \\
\bar{c}^{2}_h(f) &= \frac{|\bar{S}^h_{xy}(f)|^2}{\bar{S}^h_{xx}(f) \bar{S}^h_{yy}(f)} \\
\bar{\phi}_h(f) &= \arctan \left( \frac{\mathrm{Re} \left[ (\bar{S}^h_{xy}(f) \right]}{\mathrm{Im} \left[ (\bar{S}^h_{xy}(f) \right]} \right)
\end{align}
% \SDR{Astronomers use the symbol $\odot$ to refer to the sun, so we should probably replace it with $\star$ or $*$, depending on whether it's a cross-correlation or a convolution}
% \CLH{Noted. I was hoping to refer to a componentwise product with a taper. Are you aware of notation for a direct product? I'm finding the notation in this whole section a bit cumbersome, especially all of the $\mathcal{F}$'s. Any help is appreciated.}
\SDR{I hope this notation will make more sense to astronomers - I replaced both $\odot$ and $\angle$, which is not commonly used in our literature, and substituted $k$ for $j$ so we can keep $j$ for the time domain}

One often uses the Daniell window as a smoother (a simple moving average), or more often, the modified Daniell window which is defined as 
\begin{equation}
    % h_j = \left\{ \begin{array}{ll} \frac{1}{2m} & j = -m+1,\ldots,0,\ldots, m-1 \\
    h_k = \left\{ \begin{array}{ll} \frac{1}{2m} & k= -m+1,\ldots,0,\ldots, m-1 \\
    % \frac{1}{4m} & j = \pm m \\
    \frac{1}{4m} & k = \pm m \\
    0 & \mbox{otherwise.}\end{array} \right.
\end{equation}

\item To use the segment averaging approach, the data are first divided into overlapping blocks according to the well-known
Welch overlapped segment averaging method (WOSA) \cite{SCHULZ1997929}. Supposing there are $\ell$ data blocks and each block contains $n$ 
samples, one then denotes
the $\ell$th sub-series $\bfx^{(\ell)} = [x_{\ell}, \ldots, x_{\ell+n}]^T$, $\bfy^{(\ell)} = [y_{\ell}, \ldots, y_{\ell+n}]^T$ for $\ell = 0, \ldots, L-1$. 
When a 50\% overlap of the segments is chosen, then $L = \lfloor 2N/(n+1)\rfloor$, for example.\footnote{Note that the division of data in such a way 
implies that the different segments have different durations $T^{(\ell)} = t_{\ell+n} - 
t_{\ell}$ and different analysis bandwidths (Nyquist equivalent). The latter is often estimated as
$\bar{\Delta} t^{(\ell)} = T^{(\ell)}/n$, but is a matter of debate (and certainly makes difficult the
problem of determining aliased frequencies). Importantly, one must
ensure that the Fourier transforms computed on each segment are done in such a way that the 
frequency grid is the same.} and one computes the segment averaged MSC and phase
\begin{align} \label{eq:WOSACoh}
\bar{S}^L_{xy}(f) &= \frac{2}{\sum_{\ell} T^{(\ell)}} \sum_{\ell = 0}^{L-1} \mathcal{F}\{\bfx^{(\ell)} \otimes  \bfv\}(f) \mathcal{F}^{*}\{\bfy^{(\ell)} \otimes \bfv\}(f) \\
\bar{c}^{2}_L (f) &= \frac{|\bar{S}^L_{xy}(f)|^2}{\bar{S}^L_{xx}(f) \bar{S}^L_{yy}(f)} \\
\bar{\phi}_L(f) &= \arctan \left( \frac{\mathrm{Re} \left[ \bar{S}^L_{xy}(f) \right]}{\mathrm{Im} \left[ \bar{S}^L_{xy}(f) \right]} \right)
\end{align}
where the data taper $\bfv$ now contains $L$ data points and has unit power. The estimate is also corrected
for bias as described in \citet[\S 2.1.1]{olafsdottir16}. A false-alarm level for the coherency
is given according to the theoretical $\chi^2$ distribution for the coherence, given the {\it effective} number of segments when overlap is taken into account. 

Experience with this method has shown that due to different durations $T^{(\ell)}$ and analysis bandwidths 
for the individual segments, WOSA can achieve significantly different estimates of spectrum 
and coherence depending on the number of segments one selects. One 
also gets particularly poor estimates of the spectrum and squared coherence near the lowest
and highest frequencies estimated. For particularly perverse datasets, such as those 
encountered here, the time increments $\Delta t_j = t_{j+1}-t_{j}$ can range over orders of 
magnitude (Figure \ref{fig:HD26965_dt}). This results in the lowest frequency for segment $\ell$, $2/T_{\ell}$, and 
analysis bandwidth, $(n-1)/(2 \sum_{j = \ell}^{n+\ell-1} \Delta t_j)$, similarly having 
large variation. Clearly if one sets a single lowest and highest frequency of interest, 
the estimate computed over none of the segments will properly cover the frequency range 
of interest, being particularly bad for the low and high range.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{HD26965_dthist.pdf}
    \caption{Time increments between observations $\Delta t_j = t_j - t_{j-1}$ for $j = 2..N$ from the HD~26965 dataset presented by \citet{Diaz18}. The time increments cover more than six orders of magnitude.}
    \label{fig:HD26965_dt}
\end{figure}

\CLH{One also encounters with this routine, strange values for the phase at the origin and 
the analysis bandwidth. Since the cross-spectrum should be real at these values, the
only possibilities for the phase are $0$ and $180^{\circ}$, however this algorithm 
does not fix the endpoints, which makes for nonsense phase when the phase is ``unwrapped" to range outside
$[-180,180)$.}
\end{enumerate}

\subsection{REDFIT-X\label{sec:REDFITX}}

The method of REDFIT-X \cite{olafsdottir16}, was developed specifically for paleoclimate datasets, and 
follows the standard WOSA routine outlined above, but by assuming uncorrelated red models for both spectra, 
it promises a test for significance away from the model of red spectrum and zero coherence. The red model
is generally applied to turbulent processes in the physical sciences, and so is likely a good approximation
to the background process for astrophysical datasets.
The main assumption is that $\bfx, \bfy$ are uncoupled (i.e. the true coherence is zero) autoregressive 
processes of order 1, denoted AR(1) \cite{storchz99, pw93}. The discrete time series $x_j$ has a model equation of the form \cite{MUDELSEE2002}
\begin{equation}\label{eq:AR1model}
x_j = x_{j-1}e^{-(t_j - t_{j-1})/\tau_x} + \epsilon^x_j
\end{equation}
with initial condition $x_0$ is a standard normal random variable, the process $\epsilon^x$ is distributed
according to $\epsilon^x_j \sim N(0, 1-\exp\{-2(t_j - t_{j-1})/\tau_x\}$ for all $0<j< N$ and $\tau$ is the 
\emph{persistence time}\footnote{\CLH{I believe persistence time is the location in time of the first zero of the 
autocorrelation function. There is no value for tau that creates a white spectrum, and $\tau = \infty$ 
creates a process with a unit root and zero variance for the noise process, in which case the spectrum does not exist.}}.  

One can fit this model to the series $x_j$ by estimating the persistence time $\tau_x$ using the routine 
described in \cite{MUDELSEE2002}. To generate significance levels for the spectra, 
$M\sim 1000$ sample AR(1) spectra are generated with these 
parameters and the 95th quantile is computed from these trials at each frequency. Similarly one has $S_y(f)$ 
for the process $y(t)$, only with parameters $\tau_y$ and $y_j$ is uncorrelated with all $x, \epsilon^x$.
To compute the significance of the coherence and phase, one simulates $M$ realizations of the time series 
$y$, then generates the $95\%$ quantiles for the coherence and phase computed on the randomly generated 
processes and uses this as a threshold for significance. Note that the random realizations are uncorrelated
so represent the case where the spectra are red but have zero coherence. In the astrophysical context, 
one is interested in the locations in frequency where one exits the 95\% threshold for the red model for
the spectrum and zero coherence. Where coherences exit these limits, the estimated phase is of interest. 

\JH{We should probably insert a figure here plotting the Welch tapers computed in REDFIT-X, in both the time and frequency domain. I'm still working on generating this plot.}

\textbf{Discussion}:

\CLH{One gets poor performance from REDFIT-X when you have an oscillation frequency close to the origin and this
messes up the estimation of the persistence time and thus the whole apparatus for estimating
the significance is scuppered. One also gets poor results when one examines WOSA estimates computed with 
different numbers of tapers: a peak at one
frequency may appear to be significant when computed with some number of segments but
is no longer significant when one uses a different number of segments. }

\SDR{Charlotte: From what you've written in this section, it looks as if you're concerned that we can't get WOSA to give us reliable results. I'll defer to your judgment. Should we be writing two manuscripts in parallel, this one about multivariate techniques esp.\ coherence and another one on multitaper with gpss? With American Astronomical Society journals (ApJ and AJ), it's possible to do companion papers, i.e.\ Planet Validation in the Frequency Domain.\ I.\ Constructing Debiased, Low-variance Power Spectra with Generalized Prolate Spheroidal Sequences, and Planet Validation in the Frequency Domain.\ II.\ Coherence and Cross-spectra. We could submit the papers in tandem and request that they be reviewed together.}

\CLH{The Bronez 1992 paper \cite{bronez92} shows that the multitaper method best conserves bias, variance
and bandwidth between WOSA, multitaper, and smoothing across frequency for spectrum estimation.}

==> Input/math.tex <==


 
The spectrum of a zero-mean continuous time stationary process $x(t)$ is formally defined through 
the existence of a stationary, orthogonal increments process $dZ_x(f)$ for which 
\begin{equation} \label{eq:cramerrepn}
    x(t) = \int_{-\infty}^{\infty} e^{-i 2 \pi f t} dZ_x(f)
\end{equation}
where the integral is defined through Riemann-Stieltjes integration. Then the spectrum is the second 
moment $S_x(f) df =\mbox{E} \{|dZ_x(f)|^2\}$, \cite{cramer}. The spectrum is then the Fourier transform 
of the autocovariance function of the time series (Wiener Khintchine theorem), i.e. it partitions the 
variance of the process across 
frequency. When one has two zero mean time series $x(t)$ and $y(t)$ which are jointly stationary
one can define their \emph{cross spectrum} $S_{xy}(f) df =\EV dZ_x(f)dZ_y^*(f)\}$, where the asterisk in superscript denotes complex conjugation. 

The coherency between two zero mean jointly stationary continuous time series $x(t)$ and $y(t)$ is defined as
\begin{equation} \label{eq:coh}
  \rho(f) = \frac{S_{xy}(f)}{\sqrt{S_x(f) S_y(f)}},
\end{equation}
where $S_y(f)$ denotes the spectrum of the process $y(t)$, and $S_{xy}(f)$ denotes the (complex-valued) 
cross spectrum of $x(t)$ and $y(t)$. 

The squared magnitude of $\rho(f)$ is known as the \emph{magnitude
squared coherence} (MSC); and the angle, $\phi$, often reported in degrees, is the
\emph{phase}. The MSC can be interpreted as a frequency-dependent correlation
coefficient indicating the proportion of variance common to both series via a linear
relationship \cite{TC91,shumwaystoffer}. The real and imaginary 
parts of the cross spectrum, the \emph{cospectrum} and \emph{quadrature spectrum}, are the scaled cosine and 
sine series expansions of the product of the two time series and are large where the phase angle is 
small (also called in-phase spectrum) and large, respectively \cite{koopmans95, storchz99}.

%
% When one has a discrete, finite sample of the time series $x_j$, $j = 0, \ldots, N-1$ one estimates the 
% quantities of interest in the frequency domain using the (nonuniform) Fourier transform

%\begin{equation} \label{eq:NFFT}
%   \hat{x}(f) = \sum_{j=0}^{N-1} x_j e^{-i 2 \pi f t_j}.
%\end{equation}
%
% When the samples are equally spaced, one uses $t_j = j/\Delta t; j = 0, 1, \ldots, N-1$, where $\Delta t$ is
% the sampling rate, in time units. 



==> Input/multitaper.tex <==

\subsection{Multitaper Method\label{sec:MT}}

The Thomson multitaper method \cite{t82} was extended in 1988 to processes with unequal sampling increments
by \cite{bronez1988spectral}. The main advantage of this method is that both bias and variance can be 
constrained using frequency-dependent tapers that both constrain leakage and can be averaged to greatly reduce the variance. The method has recently been 
extended for use on astrophysical datasets by \cite{springford20}, using a simplified taper calculation 
for ease of computation, however we use the generalized taper formulation found in the original paper for 
performance reasons. The use of generalized tapers is well worth the effort; the tapers can be shown to use 
portions of data which have the right spacing to provide information about the frequency of interest, which
we show in the next section. 

\subsubsection{Generalized Prolate Spheroidal Sequences\label{sec:GPSS}}

The \emph{generalized prolate spheroidal sequences} extend the notion of maximally
bandlimited sequences, \cite{S78}, to those sampled on an irregular grid.  Define the
process half bandwidth $\beta$, analogous to the Nyquist rate for regular sampling
schemes ($\beta = 1/2$ for unit sampling), and bandwidth $W$ for the desired spectral
window, and let the sequences be given on the length $N$ index set
$\{t_n\}_{n=0}^{N-1}$. Then, following \cite{bronez1988spectral}, the orthogonal sequences
$\gpss{k}{n}{f}$ whose (nonuniform) Fourier transforms maximize the ratio of power on
$(-W, W)$ to $(-\beta, \beta)$ are solutions to the eigenvalue problem
\begin{equation} \label{eq:gpss} 
  \lambda_k(f) \sum_{m = 0}^{N-1} e^{-i2\pi f (t_n-t_m)} 
  \frac{\sin 2\pi \beta (t_n - t_m)}{\pi (t_n - t_m)} \gpss{k}{m}{f} =
  \sum_{m=0}^{N-1} \frac{\sin 2\pi W (t_n - t_m) }{\pi (t_n - t_m)} \gpss{k}{m}{f},
\end{equation}
where $\gpss{k}{n}{f}$ denotes the $k$th generalized Slepian taper at time $t_n$ and
frequency $f$ and $\lambda_k(f)$ is its associated eigenvalue. Note that both of
these explicitly depend on $N$ and $W$ but for simplicity this is suppressed in the
notation. In general, the eigenvalues and tapers are complex-valued, and the
eigenvalue problem above must be solved at each frequency of interest for use in the
spectrum estimator of \cite{bronez1988spectral}. The eigenvalues are sorted in decreasing
order $1>\lambda_0>\lambda_1>\ldots>\lambda_{N-1}>0$ and only the first $K$
tapers having large eigenvalues close to one should be used. In practice, with particularly
bad sampling, the eigenvalues can be quite far from one. 

% NEEDS AN EXAMPLE: a good taper, a relatively bad taper, the periodogram window function and a Tukey taper or something on the particular time grid we have.

By applying the nonuniform discrete Fourier transform to the generalized data taper
in \eqref{eq:gpss}, one obtains the generalized prolate spheroidal wave 
functions, or \emph{generalized Slepian functions} at the frequency $f_0$
\begin{equation} \label{eq:gpswf}
V^{k}(f; f_0) = \sum_{n = 0}^{N-1} \gpss{k}{n}{f_0} e^{-2 \pi i t_n f}
\end{equation} 
The generalized Slepian sequences form an orthonormal set on the grid
$\{t_n\}_{n=0}^{N-1}$; and the generalized Slepian functions are orthonormal on
$(-\beta,\beta)$ and orthogonal on $(-W,W)$. 

\subsubsection{Multitaper Spectrum and Coherence estimation}

In this section, $\gpss{k}{n}{f}$ for $\{t_n\}_{n=0}^{N-1}$, $k=0,\ldots,K-1$
will denote the generalized prolate spheroidal sequences computed as described in \S
\ref{sec:GPSS} on a temporal grid with unit sampling containing gaps and having
bandwidth $W$. If $\{x_n\}_{n=0}^{N-1}$ are samples from a stationary, zero mean time
series on the same grid, one constructs a multitaper estimate of the
spectrum as follows. First, one computes the \emph{eigencoefficients}
in \cite{bronez1988spectral} using the nonuniform discrete Fourier transform
\begin{equation}\label{eq:Ecoefs}
\hat{y}^{(k)}(f) = \sum_{n=0}^{N-1} \gpss{k}{n}{f} x_n e^{-i 2 \pi f t_n}.
\end{equation}
The squared magnitudes of the eigencoefficients, the \emph{eigenspectra}, are
approximately independent estimators of the power spectrum
\begin{equation} \label{eq:Sk}
\widehat{S}^{(k)}(f) = |\hat{y}^{(k)}(f)|^2.
\end{equation}
The approximate bandlimitedness of the tapers controls the bias of each
$\hat{S}^{(k)}(f)$ and each of these is exponentially distributed. One gains a
significant reduction in variance by estimating the spectrum using a weighted average
of the eigenspectra,
\begin{equation} \label{eq:Sbar}
  \widehat{S}(f) = \frac{\sum_{k=0}^{K-1} d^2(f) \widehat{S}^{(k)}(f)
}{\sum_{k=0}^{K-1} d^2(f)},
\end{equation}
where we have used $K \approx 2NW$ tapers. The frequency-dependent weights, $d(f)$,
are chosen so as to satisfy the equation \cite[\S V]{t82}
\begin{equation}\label{eq:weights}
  \sum_{k=0}^{K} \frac{\lambda_k(f)(\widehat{S}(f) - \widehat{S}^{(k)}(f))}{
    (\lambda_k(f) \widehat{S}(f) + s^2(1-\lambda_k(f))(f))^2} = 0.
\end{equation}
where $s^2 = (N-1)^{-1} \sum_{j=0}^{N-1} x_j^2$
is the sample variance of the time series. The control of the bias-variance
tradeoff through the adjustment of bandwidth is widely recognized as the main
performance advantage of the multitaper method \cite{bronez92,haley17}. A
useful quantity indicating variance reduction by the estimator is the degrees of
freedom,
\begin{equation} \label{eq:dof}
\nu(f) = 2 \sum_{k=0}^{K-1} d_k(f)^2
\end{equation} 
which is generally near $2K$ except where adaptive weighting has identified regions
in frequency where there would be high bias with equal weights.

A simple multitaper estimator for the squared coherence is computed in the following
way:
\begin{align} \label{eq:MTSimpleCoh}
\hat{c}^2(f) &= \frac{\left|\widehat{S}_{xy}\right|^2}{\widehat{S}_x(f) \widehat{S_y(f)}} \\
\widehat{S}_{xy}^{k}(f) &= \left( \sum_{t=0}^{N-1} x_t v^{k}_t e^{-i 2 \pi f t}
\right) \left( \sum_{t=0}^{N-1} y_j
v^{k}_t e^{-i 2 \pi f t} \right)^* \\
\widehat{S}_{xy}(f) &= \frac{\sum_{k=0}^{K-1} d_{xy}^2(f) \widehat{S}_{xy}^{k}(f)}{\sum_{k=0}^{K-1}
d_{xy}^2(f) },
\end{align}
where the subscripts $x$, $y$, and $xy$ denote adaptive weights and spectrum
estimates computed for the processes $x$ and $y$, and the weights are determined
by using an iteration similar to \eqref{eq:weights}. However, this estimate only avoids 
the need for smoothing \cite{brockwelldavis92} through the use of
frequency-dependent weights.
More questionable is the application of \eqref{eq:weights}, derived for univariate
spectrum estimators, to cross-spectra. Moreover, while the distributions of squared
coherence and phase are known \cite{hannan-mts, carter87, TC91}, use of
frequency-dependent weights implies frequency-dependent degrees of freedom for the
constituent cross spectra, for which these formulae do not apply.

\subsubsection{Jackknifing Multitaper Estimates}

For reasons described in \cite{TC91} and the next section, the recommended technique
for estimation of multitaper magnitude squared coherence and phase is to jackknife
over tapers, using an appropriate variance-stabilizing transformation. This
alleviates the need for smoothing and arbitrary weighting of the cross-spectrum
\cite{TC91, lee83,carter87}. The jackknife mean estimator can be shown to eliminate
the linear term in an expansion of the bias \cite{EfronStein81,Cressie81} and is
statistically efficient for computation on a small number of independent samples. The
jackknife method also provides a nonparametric estimate of the variation, from which
confidence intervals can be constructed. 

While the details of jackknifing multitaper spectrum estimates are given in \cite{TC91}, 
we summarize the estimation of missing data coherence and phase via the
jackknife here. One can obtain the independent estimators of the coherency needed
for jackknifing by having used $K$ orthogonal tapers. The use of
transformations with the jackknife is especially important when the statistics of
interest are bounded \cite[\S 5.3]{Miller74}, mainly to ensure the applicability of
the Student-$t$ distribution for the construction of the confidence intervals when
$K$ is relatively small.  For these reasons we prefer to jackknife over logarithms of
the spectrum, inverse hyperbolic tangents of the coherence, and ratios or \emph{phase
factors} computed from the phase, in order that bounded and non-normal statistics can
be closer to Gaussian. 

\subsubsection{Jackknifed Estimates of Coherence and Phase\label{sec:JkCohPhase}}

When the true coherency is zero, and there is equal spacing between samples, one can
show that the distribution of an estimate $c^2$ of the MSC based on $2K$ degrees of
freedom is \cite[p 259]{hannan-mts}
\begin{equation} \label{eq:MSCdist}
p(c^2| \gamma^2 = 0) = \frac{(1-\rho^2)^K}{K-1}(1-c^2)^{K-2} _2F_1(K,K; 1; \rho^2 c^2).
\end{equation}
where $_2F_1$ is Gauss's hypergeometric function. 
For jackknifing the MSC, the preferred transformation is an inverse hyperbolic
tangent, that is, 
\begin{equation}
Q = \sqrt{K - 2} \tanh^{-1}(|c|),
\end{equation}
which converts $|c|$ to almost Gaussian \cite{koopmans} with unit variance. One
computes the transformed jackknife MSC by denoting by $\hat{x}_k(f)$ and $\hat{y}_k(f)$ the
eigencoefficients \eqref{eq:Ecoefs} of the missing data series $x_n$ and $y_n$ and by 
computing the delete-one estimates
\begin{equation} \label{eq:jkMSCQ}
Q\subWO{j} = \sqrt{2K-2} \tanh^{-1} \left ( \frac{ \left| \sumWO{k}{j}^{K-1} 
\hat{x}_k (f) \hat{y}^*_k(f) \right|}{\sumWO{k}{j}^{K-1} |\hat{x}_k (f)|^2 \cdot 
\sumWO{k}{j}^{K-1} |\hat{y}_k (f)|^2 } \right) 
\end{equation} 
and their average
\begin{equation}
  Q \subWD = \frac{1}{K} \sum_{j=0}^{K-1} Q\subWO{j}.
\end{equation}
The jackknife mean estimate of the coherence is then 
\begin{equation} \label{eq:JkmeanCoh}
  \tilde{Q} = K\hat{Q}_{\mbox{all}} - \frac{K-1}{K} \sum_{j=0}^{K-1} 
                \hat{Q}\subWO{j},
\end{equation}
where $\hat{Q}_{\mbox{all}}$ denotes the estimate \eqref{eq:jkMSCQ} using $j=K$, i.e.
all the segments, and the variance estimate for the transformed MSC at frequency $f$ is
\begin{equation}
  \tilde{\sigma}_Q^2 = \Var Q \} = \frac{K-1}{K} \left(\hat{Q}\subWO{j}  
      - \hat{Q}\subWD \right)^2,
\end{equation}
One can construct the following two sided confidence interval for the coherence, where
$t_{K-1}(1-\alpha/2)$ denotes the Student-$t$ critical value for the significance level
$0<\alpha<1$,
\begin{equation} \label{eq:CohJKCI}
  \tanh \left(\frac{\tilde{Q} - t_{K-1}(1-\alpha/2)\tilde{\sigma}_Q}{\sqrt{K-2}}\right) 
< |c| \leq
\tanh \left(\frac{\tilde{Q} + t_{K-1}(1-\alpha/2)\tilde{\sigma}_Q}{\sqrt{K-2}}\right).
\end{equation}

For the phase estimate, we opt to compute the phase factors
\begin{equation} \label{eq:phasefact}
e\subWO{j} = \frac{\tilde{c}\subWO{j}}{|\tilde{c}\subWO{j}|}, 
\end{equation}
for $j = 0, \ldots, K-1$ and their average
\begin{equation} \label{eq:phasefactave}
e\subWD = \frac{1}{K} \sum_{j=0}^{K-1} e\subWO{j} 
\end{equation}
if $\phi\subWO{j} = \mbox{angle}(e\subWD)$, then the jackknife variance estimate is
\begin{equation} \label{eq:JkvarPhase}
\Var \phi\subWD \} = 2(K-1) (1-|e\subWD|).
\end{equation}


\subsubsection{Harmonic F-test \label{sec:Ftest}}
One of the most useful tools related to the multitaper technique is the ability to test for discrete
oscillations, or line components \cite[p. 1084]{t82}, and it relies on the extended Munk-Hasselman 
representation for the process. Using the representation \eqref{eq:cramerrepn}, for the stationary 
process $x(t)$, and extending the representation to allow for deterministic line components, write 
its first moment $\mu(f)$ as
\begin{equation} \label{eq:MunkHasselman}
\mu(f) = E\{dZ(f)\} = \sum_j \mu_j \delta(f-f_j)df
\end{equation} 
where $\delta(f)$ is the Dirac delta function, and $f_j$ are line component frequencies. The continuous part 
of the spectrum is $S(f)df = E\{|dZ(f) - E\{dZ(f)\}|^2\}$, which is simply $E\{|dZ(f)|^2$ when no harmonic 
components are present. 

Estimation of $\mu(f)$ with an unequally sampled time series can be done by minimizing the sum of squares 
distance between the eigencoefficients and their expected value. This minimization results in the following 
estimate for $\mu$
\begin{equation}\label{eq:muhat}
\hat{\mu}(f) = \frac{\sum_{k=0}^{K-1} V^{k}(0;f)\hat{y}^{(k)}(f)}{\sum_{k=0}^{K-1} |V^k(0;f)|^2}.
\end{equation}
The variance-ratio gives an $F$-distributed test statistic as 
\begin{equation}\label{eq:Fstat}
F(f) = \frac{(K-1)|\hat{\mu}(f)|^2 \sum_{k=0}^{K-1} |V^{k}(0;f)|^2}{\sum_{k=0}^{K-1} |\hat{y}^{(k)}(f) - \mu(f)V^{k}(0;f)|^2}
\end{equation}
the numerator and denominator are $\chi^2$ distributed and have $2$ and $2K-2$ degrees of freedom (df), respectively when the line frequency is known.\footnote{It is important to
adjust one's expectations, since significant F-test statistics are guaranteed to occur for $\alpha$ 
proportion of the time, testing a large number of frequencies will result in a great number of significant
frequencies. For this reason, Thomson suggests using the cutoff $\alpha = 1 - 1/M$ where $M$ is the number
of frequencies.}
$V^{k}(0;f_0)$ can be written in terms of generalized Slepian sequences, see equation \eqref{eq:gpss},
\begin{equation}\label{eq:UKzero}
V^{k}(0;f) = \sum_{n=0}^{N-1} v_n^{(k)}(f).
\end{equation}
\CLH{This section reads too concisely and needs another pass. Consider it a draft.}

\section{Examples}

\subsection{$\alpha$ Cen B asteroseismology}

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figures_multitaper/aCenB_astero_data.png}
    \caption{$\alpha$ Cen B asteroseismology data of \citet{carrier03}.}
    \label{fig:aCenB_astero_data}
\end{figure}

\begin{figure}
    \centering
    \begin{tabular}{c}
    \includegraphics[width=0.75\textwidth]{figures_multitaper/aCenB_astero_tapers.png} \\
    \includegraphics[width=0.75\textwidth]{figures_multitaper/aCenB_astero_spectralconcentrations.png} \\
    \end{tabular}
    \caption{Tapers for $f = 50$ cycles/day, spectral concentration as a function of frequency.}
    \label{fig:aCenB_astero_tapers}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figures_multitaper/aCenB_astero_powspec.png}
    \caption{Asteroseismic power spectrum of $\alpha$~Cen B.}
    \label{fig:aCenB_astero_powspec}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{figures_multitaper/aCenB_astero_ps_autocorr.png}
    \caption{Autocorrelation of asteroseismic $\alpha$~Cen B multitaper power spectrum.}
    \label{fig:aCenB_astero_ps_autocorr}
\end{figure}

==> Input/symbols.tex <==
\begin{ThreePartTable}
\renewcommand\TPTminimum{\textwidth}
% Arrange for "longtable" to take up full width of text block
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\setlength\tabcolsep{0pt}

\begin{TableNotes}
\item[a] All operators act on vectors of discrete-time data; thus, $\mathcal{F}\{\bx\}$ is a discrete or fast Fourier transform of signal $\bx$, $\bx \star \by$ is the discrete cross-correlation between signals $\bx$ and $\by$, etc.
\item[b] All time series are measured on non-uniform temporal grids.
\item[c] For the cross-spectral analysis techniques presented here, the two time series $\bfx$ and $\bfy$ must have the same temporal grid.
\end{TableNotes}

\begin{longtable}{ll}
\toprule
\caption{{\bf Symbol definitions}}
\label{tab:symbols}
\endhead

\multicolumn{2}{c}{\textit{---continued---}} \\
\endfoot

% \insertTableNotes
\endlastfoot

\multicolumn{2}{l}{\bf Operators}\tnote{a} \\
{\it Symbol     } & {\it Definition} \\
\hline
$\mathcal{F} \{ \}$ & Fourier transform \\
$\star$ & cross-correlation \\
$*$ & convolution \\
$^{T}$ & vector transpose \\
$\EV \}$ & expected value \\
$\Var \}$ & variance \\
$\otimes$ & element-wise product of two vectors \\
$\mathbf{Re}[]$ & real part of complex vector \\
$\mathbf{Im}[]$ & imaginary part of complex vector \\
\vspace{0.5cm}
\hline
\hline

\multicolumn{2}{l}{\bf Time-domain variables\tnote{b}} \\
{\it Symbol     } & {\it Definition} \\
$N$ & number of data points in each time series \\
$\bfx$ & vector containing an activity-indicator time series (e.g.\ H$\alpha$, S-index, etc.) \\
$x_j$ & $j^{\rm th}$ measurement in $\bfx$ \\
$\bfy$ & vector containing the RV time series \\
$\bfv$ & taper \\
$\tau$ & frequency-dependent time lag (see Equation \ref{eq:tau}) \\
$s_x$ & variance of time series $\bfx$ \\
$\ell$ & index of sub-series (used for Welch's algorithm, \S \ref{subsec:estimation}) \\
$L$ & number of data points in each sub-series (used for Welch's algorithm, \S \ref{subsec:estimation}) \\
$\tau_x$ & persistence time in AR(1) noise model fitted to $S_x(f)$ \\
\vspace{0.5cm}
\hline
\hline

\multicolumn{2}{l}{\bf Frequency-domain variables} \\
{\it Symbol     } & {\it Definition} \\
$f$ & frequency \\
$S_x(f)$ & power spectrum of $\bfx$ \\
$P_x(f)$ & Lomb-Scargle periodogram of $\bfx$ \\
$G(f)$ & spectral window $\mathcal{F}\{ \bfv \}(f)$ \\
$\widehat{S}_{xy}(f)$ & direct cross-spectral estimate for time series $\bfx$ and $\bfy$ (Equation \ref{eq:Crosspec})\tnote{c} \\
$h_k$  & Frequency-domain smoothing window \\
$\bar{S}^h_{x,y}(f)$ & cross-spectrum estimated via smoothing \\
$\bar{c}^{2}_h(f)$ & coherence estimated via smoothing \\
$\bar{\phi}_h(f)$ & phase spectrum estimated via smoothing \\
$\bar{S}^L_{xy}(f)$ & cross-spectrum estimated via Welch's method \\
$\bar{c}^{2}_L (f)$ & coherence estimated via Welch's method \\
$\bar{\phi}_L(f)$ & phase spectrum estimated via Welch's method \\
\hline

\end{longtable}
\end{ThreePartTable}

